CAShift: Benchmarking Log-Based Cloud Attack Detection under Normality Shift

With the rapid advancement of cloud-native computing, securing cloud environments has become an important task. Log-based Anomaly Detection (LAD) is the most representative technique used in different systems for attack detection and safety guarantee, where multiple LAD methods and relevant datasets have been proposed. However, even though some of these datasets are specifically prepared for cloud systems, they only cover limited cloud behaviors and lack information from a whole-system perspective. Another critical issue to consider is normality shift, which implies that the test distribution could differ from the training distribution and highly affect the performance of LAD. Unfortunately, existing works only focus on simple shift types such as chronological changes, while other cloud-specific shift types are ignored. Therefore, a dataset that captures diverse cloud system behaviors and various types of normality shifts is essential. To fill this gap, we construct a dataset CAShift to evaluate the performance of LAD in cloud, which considers different roles of software in cloud systems, supports three real-world normality shift types and features 20 different attack scenarios in various cloud system components. Based on CAShift, we evaluate the effectiveness of existing LAD methods in normality shift scenarios. Additionally, to explore the feasibility of shift adaptation, we further investigate three continuous learning approaches to mitigate the impact of distribution shift. Results demonstrated that 1) all LAD methods suffer from normality shift where the performance drops up to 34%, and 2) existing continuous learning methods are promising to address shift drawbacks, but the configurations highly affect the shift adaptation. Based on our findings, we offer valuable implications for future research in designing more robust LAD models and methods for LAD shift adaptation.

==> Chapters/RelatedWork.tex <==
\section{Related Work}

Benchmarking LAD

\fish{Maybe we do not need this part?}

\subsection{Dataset for Log-Based Anomaly Detection}

Many LAD datasets and methods have been proposed in existing literature. These datasets typically include normal behaviors and anomalous behaviors (including attacks) from domain-specific log systems. LAD methods learn from the normal and abnormal behaviors in these datasets and classify incoming testing logs to distinguish between normal and abnormal log activities. Specifically, LAD datasets have been discussed in certain categories including:

\noindent
\textbf{Networking Traffic Dataset.} With the rapid development of the Internet and the proliferation of Network-Based Intrusion Detection Systems (NIDS), many network traffic datasets~\cite{dragoi2022anoshift,akent-2015-enterprise-data,song2011statistical} have been proposed. Traffic datasets usually contain network packets with both normal networking logs and attacks or internal communication anomalies. Specifically, these packet logs typically include the network five-tuple and packet content for semantic analysis. Since network packets can be conveniently collected on specific ports for both normal and anomalous traffic, labeling these packets is relatively straightforward, often down to the per-log entry level.

\noindent
\textbf{System Anomaly Dataset.} For system information analysis, many datasets focus on collecting and analyzing logs extracted from systems or applications information. These datasets do not necessarily include specific attack activities but are more concerned with system robustness including internal errors and statuses. One of the most notable dataset clusters is the LogHub series~\cite{zhu2023loghub,jiang2024loghub2}. They collect system logs from various sources, including supercomputers, distributed systems, and networking servers. LogHub preprocesses these logs based on defined templates to facilitate subsequent analysis. Datasets like BGL and HDFS from LogHub are commonly used to validate existing LAD model methods. Since these log data are often manually instrumented for log collection and have pre-processing of raw data to extract clear semantic and syntactic features, the labeling for these datasets can reach a fine-grained coarse with per log entry.

\noindent
\textbf{System Attack Dataset.} Many datasets~\cite{grimmer2019modern,el2022contextualizing,lin2020cdl} are also constructed for detecting whether the systems or deployed applications are under attack. In addition to collecting normal log behaviors from the system, these datasets usually prepare vulnerable scenarios for attack replays or directly deploy the recording system or honeypots in public networks to capture real hacker intrusions. Most datasets use system calls from the system kernel as the collected log format. Unlike system anomalies such as crashes or errors, which are easy to identify through log syntax, system attack logs are difficult to perform fine-grained labeling. During the collection of attack logs, the system may still generate normal behaviors intermingled with attack activities. Moreover, many attacks (e.g., unauthorized access) resemble normal behaviors and only differ at the semantic level. Therefore, many attack datasets do not have per-log entry-level labeling, while instead, they use per-log file labeling or unfixed time-based windows for statistical analysis and detection tasks.

\noindent
\textbf{Shift-Aware Dataset.} Although most previous datasets have overlooked the issue of distribution shifts within their collection paradigms, typically maintaining a single release without considering the distribution shifts introduced over time, some datasets have acknowledged such research problems and made improvements to their collected dataset. For instance, Anoshift~\cite{dragoi2022anoshift} categorizes the yearly updated data from the Kyoto-2006+ dataset~\cite{song2011statistical} into three chronological shift patterns for evaluating the performance of network traffic-based LAD. LogHub has also expanded its collected datasets with more covered applications in LogPub~\cite{jiang2024loghub2} and provided new versions for some of the sub-datasets with new collected time versions and pre-processed templates (e.g., Hadoop, HDFS).
